VideoPhy: Evaluating Physical Commonsense for Video Generation

Recent advances in internet-scale video data pretraining have led to the development of text-to-video generative models that can create high-quality videos across a broad range of visual concepts, synthesize realistic motions and render complex objects. Hence, these generative models have the potential to become general-purpose simulators of the physical world. However, it is unclear how far we are from this goal with the existing text-to-video generative models. To this end, we present VideoPhy, a benchmark designed to assess whether the generated videos follow physical commonsense for real-world activities (e.g. marbles will roll down when placed on a slanted surface). Specifically, we curate diverse prompts that involve interactions between various material types in the physical world (e.g., solid-solid, solid-fluid, fluid-fluid). We then generate videos conditioned on these captions from diverse state-of-the-art text-to-video generative models, including open models (e.g., CogVideoX) and closed models (e.g., Lumiere, Dream Machine). Our human evaluation reveals that the existing models severely lack the ability to generate videos adhering to the given text prompts, while also lack physical commonsense. Specifically, the best performing model, CogVideoX-5B, generates videos that adhere to the caption and physical laws for 39.6% of the instances. VideoPhy thus highlights that the video generative models are far from accurately simulating the physical world. Finally, we propose an auto-evaluator, VideoCon-Physics, to assess the performance reliably for the newly released models.

==> sections/short_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\hb{mention viescore from wenhu somewhere}

\paragraph{Video Generation Models.}
Recent advancements in video generation models have emerged from two primary architectures: diffusion-based models \cite{gen2, svd, liu2024sora, blattmann2023align, wang2023lavie, wang2023modelscope, chen2024videocrafter2, khachatryan2023text2video} and autoregressive modeling-based approaches \cite{magvit2, kondratyuk2023videopoet, hong2022cogvideo, villegas2022phenaki}. Among these, diffusion models have garnered significant attention. The model known as SVD \cite{svd}, built on a latent diffusion model (LDM) \cite{ldm}, proposes a three-stage training process for video LDMs. Given the rapid development of video generation technology, our work focuses on evaluating video generation models for their physical commonsense.

\paragraph{Evaluating Video Generation Models.} Traditional evaluation methods for video generation primarily employ metrics such as FVD \cite{unterthiner2018towards} and IS \cite{salimans2016improved}. However, there is a growing consensus on the need for more comprehensive metrics to assess the performance of video generation models \cite{huang2023vbench, liu2023evalcrafter, subjectbench, lin2024evaluating}. V-Bench \cite{huang2023vbench} offers a detailed benchmark suite that introduces a hierarchical evaluation protocol with granular perspectives. Here, we propose \name{} dataset to measure the physical commonsense in the generated videos. Additionally, we introduce a \model{} auto-evaluator and analyze specific physical laws \cite{bisk2020piqa} that are violated in the generated videos through qualitative analysis. We present a detailed related work in Appendix \ref{sec:detailed_related_work}.
